Unintentional Security Flaws in Code: Automated Defense via Root Cause Analysis

Software security remains a critical concern, particularly as junior developers, often lacking comprehensive knowledge of security practices, contribute to codebases. While there are tools to help developers proactively write secure code, their actual effectiveness in helping developers fix their vulnerable code remains largely unmeasured. Moreover, these approaches typically focus on classifying and localizing vulnerabilities without highlighting the specific code segments that are the root cause of the issues, a crucial aspect for developers seeking to fix their vulnerable code. To address these challenges, we conducted a comprehensive study evaluating the efficacy of existing methods in helping junior developers secure their code. Our findings across five types of security vulnerabilities revealed that current tools enabled developers to secure only 36.2\% of vulnerable code. Questionnaire results from these participants further indicated that not knowing the code that was the root cause of the vulnerability was one of their primary challenges in repairing the vulnerable code. Informed by these insights, we developed an automated vulnerability root cause (RC) toolkit called T5-RCGCN, that combines T5 language model embeddings with a graph convolutional network (GCN) for vulnerability classification and localization. Additionally, we integrated DeepLiftSHAP to identify the code segments that were the root cause of the vulnerability. We tested T5-RCGCN with 56 junior developers across three datasets, showing a 28.9\% improvement in code security compared to previous methods. Developers using the tool also gained a deeper understanding of vulnerability root causes, resulting in a 17.0\% improvement in their ability to secure code independently. These results demonstrate the tool's potential for both immediate security enhancement and long-term developer skill growth.

==> sections/7_Survey.tex <==
Following our quantitative analysis of our model's performance, we designed a user-centric survey to evaluate the effectiveness of our proposed T5-RCGCN for assisting in code vulnerability management and educating developers in secure coding practices.

This survey comprehends an assessment that test the \textit{Assisted Group} with repairing the \textbf{SAME} five functions previously provided to the \textit{Control Group} in Subsection \ref{32_benefits_of_sota_methods} \textit{"Benefits of SOTA Techniques"}. However, different from the information provided to the \textit{Control Group}, \textit{Assisted Group} is provided with the outcomes provided by T5-RCGCN --namely,  1) the vulnerable line, 2) the CWE class with description, and 3) the vulnerability root cause. The outcomes of this survey aim to address RQ3.


%while simultaneously providing insights into the benefits and contributions of SOTA techniques.

%We analyze the qualitative result of our root cause analysis from our survey. 


%Furthermore, we categorized identified bugs according to their CWE classification \cite{cwe}.


\begin{figure}[t]
    %\begin{framed}
        \centering
        
        \includegraphics[width=0.48\textwidth]{images/survey_our.pdf}
        
    %\end{framed}
    
    \caption{Input code is depicted at the top, and output produced by our proposed system is depicted at the bottom. Input is the vulnerable code, and our system provides four types of output: 1) Identification and Classification, 2) Vulnerable Line, and 3) Root Cause.}
    \label{fig:survey_our}
\end{figure}


\subsection{RQ3: Developer Usability Evaluation}
\label{rq1}

The qualitative evaluation of the usability of our system for the \textit{Assisted Group} was based on the output of T5-RCGCN. The top box in Figure \ref{fig:survey_our} shows the vulnerable code, and the bottom box shows the root cause of the vulnerability derived from the attribution scores generated using SHAPly. This sample also presents all the other outcomes generated by our model that were provided to the \textit{Assisted Group}. Here, The vulnerability in the provided code snippet lies in the memory allocation process. Specifically, when the variable nresp (presumably, representing the number of responses) is retrieved using $packet\_get\_int()$, there is no validation to ensure a reasonable or expected value. If $nresp$ is unexpectedly large or negative, it could allocate a potentially large or negative amount of memory using $xmalloc$, which may result in a buffer overflow or vulnerability to memory corruption. An attacker could easily exploit this vulnerability to execute arbitrary code or crash the program.

A comparative analysis of the performance of the \textit{Assisted Group} was made with the performance of the \textit{Control Group}. Complete details of this comparison are presented in Table \ref{tab:qual_com_1}. By analyzing the written code from these 13\% of the participants, we found that 18\% of the code generated by ChatGPT has vulnerabilities. From this table, we can see that for each CWE, the percentage of participants in this group tasked with repairing the code compared to the control group is significantly higher for all cases. The "Repair Improvement" column from Table \ref{tab:qual_com_1} shows the improvement percentage of the participants who could repair the vulnerable code compared to the control group. From the follow-up questions after the code completion task, we found that 13\% of the participants use ChatGPT extensively for code repair. While we assumed this would be a plausible event, we still considered the outcome generated by ChatGPT in our results.

\input{tables/table_3}

Furthermore, we analyzed how long it took the participants to complete their given task. In the given code, the participants were tasked to record the start and end times when they wrote the requested code. Table \ref{tab:qual_com_1} also shows a good improvement in the percentage of the assisted participants who solved the vulnerability more quickly. For example, for CWE-20, CWE-264, and CWE-125, the participants took at least 10\% less time than their controlled counterparts. This improvement in time shows that our model can significantly boost a developer's time to repair a vulnerability by providing a root cause of the vulnerability and a static description of the CWE.

\begin{figure}[!b]
    %\begin{framed}
        \centering
        
        \includegraphics[width=0.5\textwidth]{images/learning_1.pdf}
        
    %\end{framed}
    
    \caption{Performance of Developer Education when Comparing Assisted vs. Control Group}
    \label{fig:learning_1}
\end{figure}

\paragraph{\textbf{Developer Education}} In this part, we conduct a survey with the participants of the \textit{Control Group} and the \textit{Assisted Group} to determine how our system eventually educates developers to write vulnerability-free code. it is important to note that the \textit{Control Group} has never seen an outcome from our model T5-RCGCN. Therefore, we hypothesized that by seeing the outcome from our model, the \textit{Assisted Group} had developed the ability to write more vulnerability-free code. In other words, we want to determine how self-sufficient the developers have become in fixing code vulnerabilities entirely for the participants in each group. 

To test this, we asked both participants of both groups with the same ten functions we asked them to reuse the code they completed in Subsection \ref{31_developers_proficiency_assessment}. Then, we asked both groups to check their code, and based on their learning from the previous phase, they could fix any existing vulnerabilities in their code without any assistance.

Our comparison presented in Figure \ref{fig:learning_1} shows that the participants from the \textit{Assisted Group} have a higher success rate in finding and repairing vulnerabilities from their original code across all CWE types. Furthermore, in the \textit{Control Group}, there were still vulnerabilities in 49\% of the codes they submitted after re-submission. However, in the \textit{Assisted Group}, we see only 38\% of the code has a vulnerability. Hence, we see an almost 9\% improvement in developer learning from \textit{Assisted Group} when using our system compared to SOTA techniques. Furthermore, after the survey, 42.3\% of the assisted participants responded that they feel more comfortable with analyzing and repairing source code vulnerability, compared to 34\% from the control group.










==> sections/8_Post-exposure_Assessment.tex <==


Furthermore, we asked the developers from both groups to rewrite the ten functions they wrote in the baseline stage in Subsection \ref{moti_1} to fix any possible security issues. The goal was to determine how developers from both groups improved their knowledge using SOTA techniques in the control group compared to our technique in the assisted group. This part was done in Subsection \ref{rq1}.


We described the workflow of our survey in Appendix \ref{9_appendix}.

extend the knowledge they have acquired regarding the rectification of security-related code vulnerabilities. 
we also test the capability of our model to educate the developers in writing vulnerability-free code without assistance.

Our goal is to compare the performance between the controlled and assisted in repairing the vulnerability given the outcome from SOTA techniques and the outcome from our system. 

==> sections/Table_1.tex <==
\begin{table}[ht]
\centering
\caption{Demography of the Participants from the Assisted and Controlled Group}
\begin{tabular}{lrrr}
\hline
\multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{\textbf{Control}} & \multicolumn{1}{l|}{\textbf{Assisted}} & \multicolumn{1}{l}{\textbf{Total}} \\ \hline
\multicolumn{4}{c}{\textbf{Undergraduate}}                                                                                                                               \\ \hline
\multicolumn{1}{l|}{Junior (Year 1 and 2)} & \multicolumn{1}{r|}{5}       & \multicolumn{1}{r|}{6}        & 11\\ \hline
\multicolumn{1}{l|}{Senior (Year 3 and 4)} & \multicolumn{1}{r|}{6}       & \multicolumn{1}{r|}{8}        & 14\\ \hline
\multicolumn{4}{c}{\textbf{Graduate}}                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{MS}                    & \multicolumn{1}{r|}{6}       & \multicolumn{1}{r|}{6}        & 12\\ \hline
\multicolumn{1}{l|}{PhD}                   & \multicolumn{1}{r|}{8}       & \multicolumn{1}{r|}{11}       & 19                                                  \\ \hline
\multicolumn{4}{c}{Years of Programming Experience}                                                                                                             \\ \hline
\multicolumn{1}{l|}{0-2 Years}             & \multicolumn{1}{r|}{4}       & \multicolumn{1}{r|}{7}        & 11                                                  \\ \hline
\multicolumn{1}{l|}{2-5 Years}             & \multicolumn{1}{r|}{9}       & \multicolumn{1}{r|}{13}       & 22                                                  \\ \hline
\multicolumn{1}{l|}{More than 5 Years}     & \multicolumn{1}{r|}{8}       & \multicolumn{1}{r|}{9}        & 17                                                  \\ \hline
\multicolumn{4}{c}{Security Courses Taken}                                                                                                                      \\ \hline
\multicolumn{1}{l|}{Yes}                   & \multicolumn{1}{r|}{1}       & \multicolumn{1}{r|}{2}        & 3\\ \hline
\multicolumn{1}{l|}{No}                    & \multicolumn{1}{r|}{21}      & \multicolumn{1}{r|}{32}       & 53\\ \hline
\multicolumn{1}{l|}{Total}                 & \multicolumn{1}{r|}{22}      & \multicolumn{1}{r|}{34}       & $\leftarrow$ N = 56                        \\ \hline
\end{tabular}
\label{tab:demo_moti}
\end{table}

==> sections/Table_2.tex <==
\begin{table}[t]
\centering
\caption{Success rate of participants on completing ten different functions with proper security measures}
\begin{tabular}{l|r|r}

\hline
Function Name                  &   CWE Number &     Success     \\ \hline
\texttt{calculateCombinations} &       119    &      20\%       \\
\texttt{extractPrice}          &       264    &      40\%       \\
\texttt{exportPrices}          &       125    &      22\%       \\
\texttt{*loadPrices}           &       200    &      26\%       \\
\texttt{printMaxPrice}         &       416    &      46\%       \\
\texttt{validateUserCreation}  &       399    &      33\%       \\
\texttt{addUser}               &       20     &      18\%       \\
\texttt{removeUser}            &       476    &      26\%       \\
\texttt{promptUserCreation}    &       189    &      33\%       \\
\texttt{*resizeDatabase}       &       190    &      26\%       \\ \hline
\end{tabular}
\label{tab:moti_1}
\end{table}

==> sections/Table_3.tex <==
\begin{table}[h]
\centering
\caption{The success rate of participants from the control group who could repair the function only when the vulnerable line and the CWE class of the vulnerability for each function were provided.}
\begin{tabular}{l|r|r}

\hline
Function Name               &      CWE-Number     & Success \\ \hline
\texttt{getValueFromList}   &      125        &      47\%      \\
\texttt{*callHelper}        &      416        &      48\%      \\
\texttt{SQLConnect}         &      264        &      20\%      \\
\texttt{readFile}           &      416        &      20\%      \\
\texttt{*createBoard}       &      20         &      46\%      \\ \hline
\end{tabular}
\label{tab:moti_2}
\end{table}

==> sections/backup.tex <==
%(B.1) Developers proficiency baseline: To evaluate their coding proficiency and their ability to write secure code, both groups were presented with the task to create ten code functions associated with a grocery store management system (Let's name these SQ1). For each requested code function, a skeletal code (a function declaration without implementation) was provided along with implementation instructions, parameter values, return values, and example usage. These questions were provided without any prior context of the evaluation that would be considered. 

%(B.2) SOTA Benefits: For this case, the control group made use of State of the Art (SOTA) methods, which provide as an output 1) vulnerability classification and 2) vulnerability localization, to evaluate the benefits of such models for developers to identify and fix vulnerable code. To perform this evaluation, the control group was presented with five functions (Let's name these SQ2) containing a vulnerability. Each function contained a single vulnerability associated to a single CWE. The five functions were passed to each of the of the SOTA methods (VELVET, VulChecker, and LineVul). For each function, 3 pairs of outcomes (Vulnerability class and localized vulnerable lines) were evaluated (one pair per method) aand implemented a majority vote rule to identify the best collective response. At the end, only the 5 best pairs were presented to the control group.

%As part of our motivation, we conducted an empirical study involving 56 developers majoring in Computer Science from an R1 Research University. The presented study was segmented into an initial assessment that identified the \textit{Baseline coding Proficiency} of the participants and explored the \textit{Benefits of SOTA Methods}.

As the complexity of software continues to increase \cite{alenezi2020relationship}, the significance of rigorous code security analysis in the deployment stage becomes paramount. Without such measures, we leave our systems at risk, with potential vulnerabilities wide open to threat actors. These actors can exploit backdoors, unintentionally introduced by developers, that remain within the codebase and pose a severe threat to system integrity. Proactively averting such vulnerabilities before deployment by analyzing static code testing constitutes a relatively less laborious approach, resulting in substantial savings in time and reduced economic impact. Nevertheless, recent open-source static application security analysis tools exhibit limitations in addressing detected vulnerabilities as they fail to provide actionable recommendations and comprehensive explanations supporting their decisions for the developers. To comprehend this limitation at a granular level, we looked for relevant surveys in the literature. Surprisingly, such a study was yet to be conducted. 

To identify the shortcomings and benefits that current solutions provide developers, we conducted an empirical study involving 56 participants majoring in computer science at an R1 research university. This study was divided into two parts:

\begin{itemize}
    \item \textit{Developers proficiency assessment}: Focused on evaluating developers' coding proficiency and ability to write secure code.
    \item \textit{Benefits of SOTA techniques}: Focused on evaluating the benefits of current methods for developers to classify, localize, and fix vulnerable code.
\end{itemize}


%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%
\input{tables/table_1}
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%

\paragraph{\textbf{Participant Demography}} A total of 56 participants composed of Computer Science (CS) students ranging from Bachelors in their Junior year to Ph.D. students participated in this study. The participants were randomly allocated to two distinct groups --namely, (1) \textit{Control Group} and (2) \textit{Assisted Group}. Each participant filled out a demographic questionnaire where they provided information about their educational background, programming experience, and language preference.

Approximately 70\% of all participants had more than two years of programming experience. However, only one of the 23 participants from the \textit{Control Group} had taken security-related courses, and 2 from the \textit{Assisted Group} had taken security-related courses. In addition, 5 participants from the \textit{Assisted Group} and 6 participants from the \textit{Control Group} were junior university students, and approximately 80\% were senior undergraduate or graduate (MS, PhD) students with more than two years of programming experience. Furthermore, almost 60\% of the \textit{Control Group} population and 50\% of the \textit{Assisted Group} participants are graduate students. Given their career path and goals, this study's participants represent potential students entering the software industry within a year or two. Consequently, they represent an ideal population from which we gain insights about their code security knowledge acquired from the educational system and industry experience. Further details of the participants are presented in Table \ref{tab:demo_moti}.

\paragraph{\textbf{Recruitment Process.}} The recruitment of participants took place at an R1 institution. An email invitation was sent to students in the Computer Science department. The invitation was further expanded via fliers distributed across the campus with the approval and support of the department's admin. In addition, only undergraduate and graduate students who have either completed or were currently enrolled in at least one programming language course were considered. Participants came from diverse educational backgrounds and experiences: 1) Undergraduate Students with programming experience, 2) Graduate Students without industry experience, 3) Graduate Students with industry experience, and 4) Graduate Students with research experience were selected. \textcolor{red}{From our background questionnaire, we found that approximately 41\% of our participants only use print debugging methods, a staggering 82\% of the participants use manual input test cases to test the functionality of their system, and more alarmingly, 94\% of the participants have received no training on code security. We will provide a more detailed background on the participants, the user study workflow, and the questionnaire with responses to our survey in Appendix \ref{9_appendix}. Many of these participants seek to join the industry after graduation. Their selection is strategic, considering they possess limited knowledge and training in code security and are ideal candidates for our analysis.}

\paragraph{\textbf{Compensation and Approval.}} Each participant received a compensation of US\$25 for their contribution to the study. This study involved human participants and was approved by the institution’s Institutional Review Board (IRB).

%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%
% Listing 1: Function stub sample 
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%
\lstinputlisting[style=CStyle, label={lst:listing-cpp}, caption=Sample of a function stub aimed to be completed by the participant. The completed function should be able to handle integer overflow and properly set up a base case to avoid a stack overflow if solved recursively.]{code/problem1.c}
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%

\subsection{Developers Proficiency Assessment}
\label{31_developers_proficiency_assessment}

In this first part of the study, we aim to evaluate developers' coding proficiency and ability to write secure code. All participants from the \textit{Control Group} and \textit{Assisted Group} participated in this part of the study to quantify the percentage of participants from both groups who could write functional and vulnerability-free code without the assistance of any tool. Toward this objective, we crafted a careful selection of 10 function stubs written in C, which are built in reference to a grocery store management system. A function stub, also known as a method stub, serves as a preliminary model for a function in software development. Function stubs define the function's signature but contain minimal or no implementation. They are commonly used for prototyping and outlining program structure, allowing development to proceed in parallel among different system components. Each function stub was intentionally designed so participants' responses may fall susceptible to one particular type of vulnerability. The code snippet in Listing \ref{lst:listing-cpp} demonstrates one of ten function stubs participants needed to complete, covering core C programming concepts such as file I/O and memory management. This function takes a long integer parameter; any form of integer declaration will cause an Integer Overflow Wraparound (CWE-190) error during testing. Similarly, other functions are designed to potentially encounter Null Pointer dereference (CWE-476), Divide by Zero (CWE-369), and similar issues. 

It is important to note that no code security requirement was requested from the participants at this stage. This was done to observe the participants' unbiased natural coding style and code development quality to properly set a baseline reflecting their natural coding practices and their considered security measures. The participants were tasked to download the 10 C function stubs. Each function stub included implementation instructions, details of parameter values, details of return values, and usage samples. All participants were required to document each function's start and development completion times. 

%Listing \ref{lst:listing-cpp} illustrates one of the 10 function stubs the participants were required to complete. The tasks involved core C programming concepts, including file I/O and memory management. 

\textcolor{red}{This paragraph may be removed if space is short}However, the study ensured that the implementations of these functions steered clear of advanced data structures to avoid unnecessary complexity. Essential C libraries and user-defined structures were provided with the function stubs beforehand. Participants were neither encouraged nor discouraged from making use of online resources, including Generative AI or a specific Integrated Development Environment (IDE)




%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%
%\input{sections/Table_2}
\input{tables/table_2}
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%

Table \ref{tab:moti_1} presents the results pertaining to the first part of this study. In this table, we define success rate as the percentage of participants who wrote a working function without introducing the possibly associated vulnerability. It can be observed from this table that out of the 10 completed functions (based on the function stubs) submitted by each of the 56 participants, the function stub that had the lowest success rate was the function associated with CWE-119, with a success rate of 20\% and CWE-20 with a success rate of 18\%. The success rate on the remaining completed functions associated with other CWEs was slightly higher peaking at 46\% for CWE 416. The completed functions with the lowest success rate are associated with writing data outside defined memory buffer or performing improper input validation. This low performance in writing correct and secure code exhibits participants' indifference to safeguarding some of the variables used in these functions. 


\subsection{Benefits of SOTA Techniques}
\label{32_benefits_of_sota_methods}

The second part of this study was restricted to the \textit{Control Group} with the objective of systematically analyzing the benefits of publicly available SOTA techniques used to assist in secure code development. Various popular static code analysis tools were considered including Infer \cite{infer} and Cppcheck \cite{cppcheck} or deep learning methods to detect \cite{zhou2019devign} \cite{islam2023unbiased}, localize \cite{fu2022linevul} \cite{pornprasit2022deeplinedp} \cite{mirskyvulchecker} and repair \cite{fu2022vulrepair} \cite{pearce2023examining}, all of which could be used to address the security challenges faced by developers. While these tools and techniques provide some information to classify and localize vulnerabilities, they are not designed to act as an assistive/interactive tool for humans to understand detected vulnerabilities in the code. Furthermore, none of these techniques provide transparency to track down the main contributors of the model's decision. The ideal goal of such tools should not be to offload a developer's task completely but to act as an assistive tool that would educate developers with appropriate security knowledge to help them become more self-sufficient in writing secure code.

To understand the level of assistance provided by SOTA techniques help developers, participants in the \textit{Control Group} were given a second coding exercise in which they were provided with five new vulnerable code functions. Differently from the assignment used to determine the baseline, this time they were provided with information similar to the one is provided by SOTA techniques including VELVET \cite{ding2021velvet}, VulChecker \cite{mirskyvulchecker}, and LineVul \cite{fu2022linevul}. Specifically, the participants were provided with 1) the CWE classification of the vulnerability detected in the code, and 2) the line/lines of code where the vulnerability was found. A sample of this information is presented in Figure \ref{fig:survey_sota}. Each of the five vulnerable functions was processed using each of the SOTA techniques to obtain the CWE classification and the vulnerable lines. Our security experts then analyzed the outcomes for each function and selected the most accurate output pairs for each vulnerable function. This approach was taken to remove any false positives or false negatives from the information given to the participants. Given this information along with the code functions, the participants were tasked to fix the vulnerability in the given code. After all participants submitted their responses, we calculated the percentage of the participants that successfully repaired the vulnerable code. 
 
 %%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%
 \begin{figure}[t]
        \centering
        \includegraphics[width=0.48\textwidth]{images/survey_SOTA.pdf}
    \caption{Sample source code provided to the participants depicted at the top and output at the bottom provided by the SOTA techniques. We conducted our initial survey by providing the participants with this information and determined their capability to repair vulnerability using these two outputs: classification and vulnerable line.}
    \label{fig:survey_sota}
\end{figure}
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%

\subsection{Code Assessment and Results}
\textcolor{red}{Assessment is propagated for later user study as well. Mention clearly}
The code assessment consisted of two evaluations, namely, 1) Run-time Analysis and 2) Manual Analysis. The first helps us evaluate the functionality of each code sample submitted by the participants while the second helps is determining the existence of any security vulnerability within the submitted code sample. 

\paragraph{\textbf{Run-time Analysis}} The Run-time analysis consisted of two sets of test cases that had to be completed by participants for each test function. The first set aimed at evaluating the functionality, ensuring that the code meets the intended requirements. The second involved analyzing the code to unveil any potential vulnerabilities accidentally crafted by the participants that could produce run-time errors.

\textcolor{red}{Might delete the following paragraph}
\paragraph{\textbf{Manual Analysis}} While most participants submitted a fully working code, some provided partially written non-compilable code. Furthermore, some participants also use pseudocode as a solution to vulnerability. Therefore, a manual code review was conducted by our internal security experts to identify potential vulnerabilities and fixes. Our security experts initially manually checked the functionality by reading code and estimated the outcome based on some input test cases. Furthermore, for security testing, our security experts checked whether the function would fall into a runtime error in the case of NULL, negative, or overloading numerical limits in the code. Based on the partially written code or pseudocode, if the function is possibly breaking at these inputs, the security experts deem it as a vulnerable function.

%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%
%\input{sections/Table_2}
\input{tables/table_2.5}
%%%%% %%%%% %%%%% %%%%% %%%%% %%%%% %%%%%

The results presented in Table \ref{tab:moti_2} shows that a majority of participants could not fix the given vulnerable code function with the provided information. While the classification and localization provided some amount of insight on the code vulnerability to the participants, we can safely assume, based on the participants' responses, that SOTA techniques helped to solve less than 50\% of the vulnerabilities. While this is an improvement compared to writing code without any suggestions, if we consider a real-world situation, we see a possibility that approximately 50\% of code in production is still susceptible to vulnerability. These results support the suggestions from recent research works that underscore the necessity of providing comprehensive security support and training to empower software developers in effectively mitigating the security issues before code deployment \cite{green2016developers, acar2016you}. Another study by Assal et al. \cite{assal2019think} delved into the human aspect of source code security, shedding light on the insufficient collaboration between software developers and security experts.

Participants were provided with four types of information based on which group they were assigned to: 1) the specific vulnerable line(s) of code, 2) the vulnerability category, 3) the description of the category, and 4) the root cause of the vulnerability.

\subsection{Concluding the Findings}

While we investigated the challenges of current SOTA techniques to identify the benefits these provide to developers, we also proceeded to asked them a list questions to identify the missing elements that could proper assist the developer in writing secure code. Participants in this study were provided with structured questions followed by an open-ended interview to determine what type of system they expected from which they would benefit the most. We also took into consideration the exposure participants had to SOTA techniques.

In the first question, we wanted to determine the number of participants familiar with CWE vulnerability categories and found that only 17\% of participants are familiar. In the following question, we decided to investigate whether they looked for the definitions or the descriptions of the CWE on the internet, and 26\% of the participants did not. Furthermore, approximately 68\% mentioned that the description would help them greatly instead of looking it online. The last question we asked the participants was an open-ended asking for the reason that could not solve the vulnerability given the information. Almost 62\% of the participants responded that they did not know which line to look for to fix the particular vulnerability. Furthermore, 66\% of the participants also mentioned that it would be of great benefit to be presented with the vulnerability line or the root cause line they have to edit to repair along with the description.

This initial study demonstrates the lack of developer training on code security. Further, it highlights the failure of current SOTA techniques in assisting developers in repairing vulnerabilities. From the open-ended interview with the participants, we concluded that it would be of great benefit to participants to be provided with system that presents them with the root cause of the vulnerability with a reasonable description of the vulnerability.



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\begin{tabular}{@{}l|l@{}}
\toprule
\textbf{CWE Number}                                                              & \textbf{Description}                                                                                                                                                                                                                                                                                 \\ \midrule
CWE-119: Improper Restriction of Operations within the Bounds of a Memory Buffer & The product performs operations on a memory buffer, but it can read from or write to a memory location that is outside of the intended boundary of the buffer.                                                                                                                                       \\
CWE-264: Permissions, Privileges, and Access Controls                            & Weaknesses in this category are related to the management of permissions, privileges, and other security features that are used to perform access control.                                                                                                                                           \\
CWE-125: Out-of-bounds Read                                                      & The product reads data past the end, or before the beginning, of the intended buffer.                                                                                                                                                                                                                \\
CWE-200: Exposure of Sensitive Information to an Unauthorized Actor              & The product exposes sensitive information to an actor that is not explicitly authorized to have access to that information.                                                                                                                                                                          \\
CWE-416: Use After Free                                                          & Referencing memory after it has been freed can cause a program to crash, use unexpected values, or execute code.                                                                                                                                                                                     \\
CWE-399: Resource Management Errors                                              & Weaknesses in this category are related to improper management of system resources.                                                                                                                                                                                                                  \\
CWE-20: Improper Input Validation                                                & The product receives input or data, but it does not validate or incorrectly validates that the input has the properties that are required to process the data safely and correctly.                                                                                                                  \\
CWE-476: NULL Pointer Dereference                                                & A NULL pointer dereference occurs when the application dereferences a pointer that it expects to be valid, but is NULL, typically causing a crash or exit.                                                                                                                                           \\
CWE-189: Numeric Errors                                                          & Weaknesses in this category are related to improper calculation or conversion of numbers.                                                                                                                                                                                                            \\
CWE-190: Integer Overflow or Wraparound                                          & The product performs a calculation that can produce an integer overflow or wraparound, when the logic assumes that the resulting value will always be larger than the original value. This can introduce other weaknesses when the calculation is used for resource management or execution control. \\ \bottomrule
\end{tabular}
\end{table*}


==> sections/summary.tex <==
In this paper, we propose a model named T5-GCN for detection, classifying, and localizing vulnerability in source code as well as identifying the root cause of the vulnerability. The main objective of this model is to assist developers in detecting and classifying vulnerabilities in source code as well as to localize the vulnerable lines and identify the root cause of the vulnerability. Our paper's contributions can be divided into two factions:

Abstract - Language and Structure Rev 4
Introduction - Language and Structure Rev 2
Related Works - Complete
Motivation: B.1-B.2 (Humans) - Complete
Preliminaries (Tentative)
Methodology: Architecture (Arch) - Complete (Language Rev 1)
Experiments: A.1 (Performance/No-Humans)
Generalizability: A.2-A.3 (Performance/No-Humans)
Survey (Main Contribution): B.3-B.4 (Humans)



(A) Contributions with respect to our model's performance and capabilities: 

(A.1) T5-GCN Performance: In this case we seek to measure the model's performance in terms of  vulnerability classification (performance metrics: accuracy, precision, recall, and F1-Score) across 10 categories (CWEs), vulnerability localization (performance metric: IoU), and identification of the root cause of the vulnerability

(A.2) T5-GCN Generalizabiity: This case is more related to the model's performance and does not involve the participants in the control or assisted group. In this case, we want to test the model's generalization capability by training the model with one dataset (i.e. D2A dataset) and testing the model's performance with another dataset (i.e. BigVul dataset) . We also did the opposite combination, training the model with one dataset (i.e. BigVul dataset) and testing the model's performance with another dataset (i.e. D2A dataset). We also combined the D2A and BigVul and then test its performance agains the D2A dataset, BigVul Dataset, and the Combined.

(A.3) T5-GCN N-Day and Zero-Day vulnerability detection: This last case is more related to the model's performance and does not involve the participants in the control or assisted group. In the first part of this case, we seek to evaluate T5-GCN performance to Detect and Classify N-day Vulnerabilities as well as to Localize the vulnerable code lines in real-world code repositories (i.e. TinyOS, Contiki, Zephyr, FreeRTOS, RIOT-OS, and Raspberry-Pi OS). In the second part, we seek to evaluate T5-GCN performance to Detect and Classify Zero-day Vulnerabilities as well as to Localize the vulnerable code lines in two code sample from Zephyr and one code sample from FreeRTOS. The three of them were CWE-119 vulnerabilities.

(B) The main contribution of this paper which are the benefits that T5-GCN can produce for developers with minimum security knowledge in recognizing vulnerabilities in code (via the detection and classification feature) and fixing the vulnerable (via the localization of vulnerable lines and root cause identification features). To identify these benefits, we gathered a 56 students (Table presented below in Latex format) and divided them into 2 groups --namely, the Control Group and the Assisted Group. The control group was composed of 22 students and the Assisted group of 34 students. For this contribution we delineated the following objectives:

(B.1) Developers proficiency baseline: To evaluate their coding proficiency and their ability to write secure code, both groups were presented with the task to create ten code functions associated with a grocery store management system (Let's name these SQ1). For each requested code function, a skeletal code (a function declaration without implementation) was provided along with implementation instructions, parameter values, return values, and example usage. These questions were provided without any prior context of the evaluation that would be considered. 

(B.2) SOTA Benefits: For this case, the control group made use of State of the Art (SOTA) methods, which provide as an output 1) vulnerability classification and 2) vulnerability localization, to evaluate the benefits of such models for developers to identify and fix vulnerable code. To perform this evaluation, the control group was presented with five functions (Let's name these SQ2) containing a vulnerability. Each function contained a single vulnerability associated to a single CWE. The five functions were passed to each of the of the SOTA methods (VELVET, VulChecker, and LineVul). For each function, 3 pairs of outcomes (Vulnerability class and localized vulnerable lines) were evaluated (one pair per method) aand implemented a majority vote rule to identify the best collective response. At the end, only the 5 best pairs were presented to the control group.

(B.3) T5-GCN Benefits: For this case, the assisted group made use T5-GCN to evaluate the benefits of our method for developers to identify and fix vulnerable code. The developers in this group were presented with SQ2 and the output provided by T5-GCN for each of the functions --namely, 1) vulnerability classification, 2) vulnerable lines (localization), and 3) vulnerability root cause. 

(B.4) Post-Exposure Assessment: After exploring the benefits of SOTA methods (fro the control group) and our proposed T5-GCN method (for the assisted group), the participants from each group were tasked to re-write the SQ1 functions. The goal of this assessment is to evaluate participants' improvement on code development in terms of functionality and code development in terms of security.

==> tables/table_2.tex <==
\begin{table}[t]
\centering
\caption{Success rate of participants on completing ten different functions with proper security measures}
\begin{tabular}{l|r|r}

\hline
Function Name                  &   CWE Number &     Success     \\ \hline
\texttt{calculateCombinations} &       119    &      20\%       \\
\texttt{extractPrice}          &       264    &      40\%       \\
\texttt{exportPrices}          &       125    &      22\%       \\
\texttt{*loadPrices}           &       200    &      26\%       \\
\texttt{printMaxPrice}         &       416    &      46\%       \\
\texttt{validateUserCreation}  &       399    &      33\%       \\
\texttt{addUser}               &       20     &      18\%       \\
\texttt{removeUser}            &       476    &      26\%       \\
\texttt{promptUserCreation}    &       189    &      33\%       \\
\texttt{*resizeDatabase}       &       190    &      26\%       \\ \hline
\end{tabular}
\label{tab:moti_1}
\end{table}
